Spin injection and emission helicity switching in a 2D perovskite/WSe2 heterostructure

The initialization and control of a long-lived spin population in lead halide perovskites are prerequisites for their use in spintronic applications. Here, we demonstrate circular polarization of the interlayer exciton emission in a (BA)2PbI4/WSe2 monolayer heterostructure. The helicity of this emission is controlled by tuning the energy of the excitation laser through the manifold of exciton resonances of the WSe2 monolayer, together with an emerging interlayer absorption feature of the heterostructure. Theoretical calculations show that this resonance arises from hybridized (BA)2PbI4/WSe2 states in the valence band. This hybrid character enables its observation in both linear absorption and ultrafast pump-probe spectroscopies, and plays a key role in controlling the sign of the helicity of the interlayer exciton emission. The tunable spin polarization demonstrated here, with the WSe2 monolayer effectively acting as a tunable spin filter, represents an important step toward the use of 2D perovskites in opto-spintronic applications.

==> latexmkrc <==
$sub_doc_output = 'output-subdoc';

@sub_doc_options = ();

push @sub_doc_options, '-pdf'; # Use pdflatex for compilation of external documents.
# Replace '-pdf' by '-pdfdvi', 'pdfxe', or 'pdflua' if needed.

push @file_not_found, '^No file\\s*(.+)\s*$';

add_cus_dep( 'tex', 'aux', 0, 'makeexternaldocument' );
sub makeexternaldocument {
    if ( $root_filename ne $_[0] )  {
        my ($base_name, $path) = fileparse( $_[0] );
        pushd $path;
        my $return = system "latexmk",
                            @sub_doc_options,
                            "-aux-directory=$sub_doc_output",
                            "-output-directory=$sub_doc_output",
                            $base_name;
        if ( ($sub_doc_output ne ' ') && ($sub_doc_output ne '.') ) {

             rdb_add_generated( "$sub_doc_output/$base_name.aux" );
             copy "$sub_doc_output/$base_name.aux", ".";
        }
        popd;
        return $return;
   }
}
